Weakly Supervised Disentanglement with Guarantees

Learning disentangled representations that correspond to factors of variation in real-world data is critical to interpretable and human-controllable machine learning. Recently, concerns about the viability of learning disentangled representations in a purely unsupervised manner has spurred a shift toward the incorporation of weak supervision. However, there is currently no formalism that identifies when and how weak supervision will guarantee disentanglement. To address this issue, we provide a theoretical framework to assist in analyzing the disentanglement guarantees (or lack thereof) conferred by weak supervision when coupled with learning algorithms based on distribution matching. We empirically verify the guarantees and limitations of several weak supervision methods (restricted labeling, match-pairing, and rank-pairing), demonstrating the predictive power and usefulness of our theoretical framework.

==> figures/label/corrplot_single_l_shapes3d.tex <==
\begin{figure}[t]
\centerline{\includegraphics[width=\textwidth]{images/label/corrplot_single_l_shapes3d.pdf}}
\caption{Correlation plot and scatterplots demonstrating the empirical relationship between $\tilde{c}(i)$ and $\tilde{r}(i)$ across all models trained via single-factor labeling on Shapes3D.}\label{fig:label_corrplot}
\end{figure}

==> figures/match/boxplot_intersect_c.tex <==
\begin{figure}[!h]
\centerline{\includegraphics[width=\textwidth]{images/match/boxplot_intersect_c_shapes3d_filter=False.pdf}}
\caption{We trained $16$ distinct models for each change-pairing intersection setup and measured the restrictiveness of each model against each factor. Our theory predicts each boxplot highlighted in red to achieve the highest restrictiveness.}\label{fig:intersect_main}
\end{figure}

==> figures/match/boxplot_match_mig.tex <==
\begin{figure}[!h]
\centerline{\includegraphics[width=\textwidth]{images/match/boxplot_match_mig.pdf}}
\caption{Disentanglement performance of vanilla GAN, fully-labeled GAN, and GANs trained on either complete-share-pairing or complete-change-pairing.}\label{fig:match_mig}
\end{figure}

==> figures/match/boxplot_single_match_shapes3d.tex <==
\begin{figure}[!h]
\centerline{\includegraphics[width=\textwidth]{images/match/boxplot_single_s_shapes3d.pdf}}
\caption{We trained $32$ distinct models for each share-pairing setup and measured the consistency of each model against each factor. Our theory predicts each boxplot highlighted in red to achieve the highest consistency.}\label{fig:match_share}
\centerline{\includegraphics[width=\textwidth]{images/match/boxplot_single_c_shapes3d.pdf}}
\caption{We trained $32$ distinct models for each change-pairing setup and measured the restrictiveness of each model against each factor. Our theory predicts each boxplot highlighted in red to achieve the highest restrictiveness.}\label{fig:match_change}
\end{figure}

==> figures/match/scatterplot_cs_shapes3d.tex <==
\begin{figure}[!h]
\centerline{\includegraphics[width=\textwidth]{images/match/scatterplot_cs_remove_outlier=True_shapes3d.pdf}}
\caption{Scatterplots of $\tilde{c}(i)$ versus $\tilde{r}(i)$ that compares the effect of using share-pairing, change-pairing, or both to train the models. In the first four plots, we see that combining share and change-pairing leads to models with the highest consistency and restrictiveness.}\label{fig:scatter_cs_shapes3d}
\end{figure}


==> figures/rank/boxplot_rank_mig.tex <==
\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{images/rank/boxplot_rank_mig.pdf}}
\caption{Disentanglement performance of vanilla GAN, fully-labeled GAN, and GANs trained on complete-rank-pairing.}\label{fig:rank_mig}
\end{figure}

==> figures/rank/boxplot_single_r_shapes3d.tex <==
\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{images/rank/boxplot_single_r_shapes3d.pdf}}
\caption{We trained $32$ distinct models for each rank pairing setup and measure the consistency of each model against each factor. our theory predicts each boxplot highlighted in red to achieve the highest consistency.}\label{fig:single_r_shapes3d}
\end{figure}

==> iclr2020_instructions.tex <==
\section{Submission of conference papers to ICLR 2020}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2020 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2020_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2020_conference.sty+ and \verb+iclr2020_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2020_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

The recommended paper length is 8 pages, with unlimited additional pages for
citations.  There will be a strict upper limit of 10 pages for the main text.
Reviewers will be instructed to apply a higher standard to papers in excess of 8
pages.  Authors may use as many pages of appendices (after the bibliography) as
they wish, but reviewers are not required to read these.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress 
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x){,}g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL{P}{Q} $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .pdf graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/00_readme.tex <==
\section{\color{red}Please Read Me}
\begin{enumerate}
\item Please use \verb|\enc| and \verb|\gen| instead of $e$ and $g$ in the document. This is so that we can easily swap notation later if need be.
\item Each major section can be found in the \verb|sections| folder. \RS{Unfortunately, this breaks double-clicking on the PDF viewer. But hopefully the gains in organization is worth it.}
\item Figures are placed in the \texttt{figures} folder as individual files and included via \verb|\input{}|.
\item Tables are placed in the \texttt{tables} folder as individual files and included via \verb|\input{}|.
\item Place all images in the \texttt{images} folder.
\item Appendix will go to \texttt{appendix.tex}. 
\item All equation/figure/table/etc references are done using \verb|\cref|.
\item Use \verb|\citep| to cite in parentheses, e.g. \citep{shu2018rethinking}. When referring to a citation as the subject of a sentence, use \verb|\citet|, e.g. \citet{shu2018rethinking} wrote a paper on disentanglement that no one read.
\end{enumerate}

==> sections/30_calculus_backup.tex <==
\section{A Calculus of Disentanglement}\label{sec:calculus}

A key feature of consistency and restrictiveness is that they operate over \emph{sets} of latent variables and factors of variation. A natural question that arises is whether consistency or restrictiveness over certain sets of variables imply additional properties over other variables. This is section, we shall develop a calculus that allows one to use consistency and restrictiveness as the basic building blocks to reason about the relationship between the latent variables and the factors of variation.

\Cref{fig:consistency,fig:restrictiveness} already provide a preliminary demonstration of the calculus, illustrating that consistency $C(I)$ and restrictiveness $R(I)$ do not imply each other. 

\input{figures/calculus/calculus.tex}
As \cref{fig:consistency} and \cref{fig:restrictiveness} illustrate, a generator consistent with respect to some factor of variation is not necessarily restrictive with respect to the same factor; vice versa. We now derive a calculus of disentanglement intended as toolbox to formally reason about properties satisfied by a certain generator or encoder. We focus on generator-based definitions, i.e., $(C, R, D) = (C_\gen, R_\gen, D_\gen)$; all rules apply to decoder-based definitions analogously. Concretely, $\gen$ has $n$ latent variables $Z_{1:n}$ and nuisance variable $z_0$.  Let $[n]$ denote index set $\{0, 1, \dots, n\}$. $I, J$ are arbitrary subsets of $[n]$. Let $L = I \cap J $,$K = \sm \left( I \cup J \right)$, $M = I - L $,$N = J - L$.

We make the following assumptions:
\RS{Assume here that types match}
\RS{In fact... apply all assumptions symmetrically? Hmm}
%YC: Yes let's apply all assumptions symmetrically.}
\begin{enumerate}
    \item We allow a subset of hidden variables to have discrete distribution and others to have continuous conditional distribution for each set of values in the support of the discrete hidden variables. Formally, let $D = \{i: z_i \text{ is discrete}\}$. Let $\mathcal{Z}_D$ be the support of $p(z_D)$. Assume:
    \begin{enumerate}
        \item $p(z_{\sm D} | z_{D})$ exists, and is continuous.
        \item Let $\mathcal{Z}(z_D) \subseteq \mathbb{R}^{|\sm D|}$ denote the support of $p(z_{\sm D} | z_{D})$. $\enc_{i}^* \circ \gen$ is continuous on $\mathcal{Z}(z_D)$ for all $i \in {\sm D}$.
    \end{enumerate}
    
    \item $\forall z_D \in \mathcal{Z}_D$, let $\mathcal{Z}(z_D)-\delta \mathcal{Z}(z_D)$ denote the interior of $\mathcal{Z}(z_D)$. Let $\mathcal{Z} = \cup_{z_D \in \mathcal{Z}_D}{\left(\left(\mathcal{Z}(z_D)-\delta \mathcal{Z}(z_D)\right) \times \{z_D\}\right)}$. Note that $\mathcal{Z} \subseteq \mathbb{R}^{n}$. We assume $\mathcal{Z}$ is {\em zig-zag path connected} \footnote{This assumption is necessary for restrictiveness union and consistency intersection. See Appendix.}, i.e., $\forall (z_M, z_L, z_N, z_K), (z_M', z_L', z_N', z_K) \in \mathcal{Z}$, there exists path $\{(z_M^t, z_L^t, z_N^t, z_K)\}_{t=0}^T$ such that
\begin{align}
    (z_M^0, z_L^0, z_N^0, z_K) = (z_M, z_L, z_N, z_K). \\
    (z_M^T, z_L^T, z_N^T, z_K) = (z_M', z_L', z_N', z_K). \\
    \forall 0 \le t <= T, (z_M^T, z_L^T, z_N^T, z_K) \in \mathcal{Z}. \\
    \forall 0 \le t < T, \text{either } z_N^t = z_N^{t+1} \text{ or } z_M^t = z_M^{t+1}.
\end{align}
\end{enumerate}
Under those assumptions, the calculus can be derived.

We give intuitions on the rules specified by the calculus (see Appendix for proofs):
\begin{enumerate}
    \item Consistency and Restrictiveness: Pictorial counterexamples for 1 and 2 are given in \cref{fig:consistency} and \cref{fig:restrictiveness}. Fixing $z_I$ fixes $s_I$ means changing $z_{\sm I}$ only changes $s_{\sm I}$.
    \item Union Rules: 1. If fixing $z_I$ fixes $s_I$ and fixing $z_J$ fixes $s_J$, then fixing $(z_I, z_J)$ should fix $(s_I, s_J)$; 2. If changing $z_I$ is restricted to changing $s_I$ and changing $s_J$ is restricted to changing $s_J$, then changing $(s_I, s_J)$ is restricted to changing $(s_I, s_J)$.
    \item Intersection Rules: 1. If fixing $z_I$ fixes $s_I$ and fixing $z_J$ fixes $s_J$, then fixing $(z_I, z_J)$ should fix $(s_I, s_J)$; 2. If changing $z_I$ is restricted to changing $s_I$ and changing $s_J$ is restricted to changing $s_J$, then changing $(s_I, s_J)$ is restricted to changing $(s_I, s_J)$.
    \item Full disentanglement: 1 and 2 follow from repeated application of intersection rules.
\end{enumerate}

The calculus is useful in both theoretical analysis and practical applications. For example,
\begin{enumerate}
    \item Dealing with nuisance variables.
    \item Experimental design: set intersection experiments, common cause.
\end{enumerate}

==> sections/55_restricted.tex <==
\subsection{Restricted Labeling}\label{sec:restricted}

We begin our analysis with weak supervision via what we refer to as restricted labeling. Formally, we say that a data-collection strategy is restricted to labeling a subset of factors $I$ if $\strat$ returns the distribution $p^*(x, s_I)$, which simply marginalizes out $s_{\sm I}$ from the following data-generation process
\begin{align}
    s_I &\sim p^*(s_I)\\
    s_{\sm I} &\sim p^*(s_{\sm I} \giv s_I)\\
    x &= g^*(s_{I}, s_{\sm I}).
\end{align}
We note that restricted labeling is distinct from semi-supervised learning; whereas restricted labeling \emph{fully} labels a \emph{subset} of the factors, the semi-supervised learning provides \emph{missing-at-random labeling} for \emph{all} the factors. The appeal of restricted labeling stems from the belief that by labeling the factor $s_i$, it is possible to learn a generative model where $z_i$ \emph{disentangles} $s_i$. This belief features prominently in the style-content disentanglement literature \citeme{kingma, style-content speech, static-motion video disentangle, pose-content disentanglement}. As we shall see, however, labeling the factors $s_I$ guarantees that $z_I$ is \emph{consistent} with $s_I$, but not necessarily restricted to $s_I$.


Since restricted labeling directly exposes the learning algorithm to the underlying factors $s_I$, it is perhaps not surprising that \Cref{thm:restricted} is true. And consistent with what is already practiced in the literature, \Cref{thm:restricted} suggests to train a generative model via distribution-matching on the observed variables. To demonstrate \Cref{thm:restricted} empirically, we trained generative adversarial networks (GANs) on six different restricted-labeling setup of the Shapes3D dataset (one setup for the restricted labeling of each factor), and then learned encoders that approximately inverted each generative model. We then measured the consistency of each encoder with respect to each factor. \Cref{fig:label_boxplot} shows our measurement of a \emph{normalized consistency score}, which we define as
\begin{align}
    \tilde{c}(I \scolon p^*, \gen^*, e) = 
    1 - 
    \frac
    {\Expect_{p^*_I} \| e_I \circ \gen^*(s_I, s_{\sm I}) - e_I \circ \gen^*(s_I, s_{\sm I}')\| }
    {\Expect_{s_{1:n}, s_{1:n}' \simiid p^*} \| e_I \circ \gen^*(s_{1:n}) - e_I \circ \gen^*(s'_{1:n})\| }
\end{align}
This score is bounded on the interval $[0, 1]$ and is maximal when $C(I \scolon p^*, \gen^*, e)$ is satisfied. This normalization procedure is similar in spirit to that used in \citet{suter2018interventional}'s Interventional Robustness Score. The normalized restrictiveness score $\tilde{r}$ can be analogously defined. Consistent with our theory, \Cref{fig:label_boxplot} shows that consistency for factor $s_i$ is highest when the model is explicitly trained with labeling of $s_i$.

\input{figures/label/boxplot_single_l_shapes3d.tex}
\input{figures/label/corrplot_single_l_shapes3d.tex}

Although \cref{thm:impossible} states that restricted labeling does not guarantee restrictiveness in theory and our calculus argues that consistency and restrictiveness do not imply each other, it is still worth determining the extent to which consistency and restrictiveness are correlated in practice. In \Cref{fig:label_corrplot}, we measured the consistency and restrictiveness of each model on each factor and provide both the correlation plot and scatterplots of $\tilde{c}(i)$ versus $\tilde{r}(i)$. Our results show that while there exists models that achieve high consistency but not restrictiveness (and vice versa), the correlation is nevertheless quite strong, and models that achieve very high consistency also tend to achieve high restrictiveness. Based on our theoretical framework, we can definitively conclude that the achieving of high restrictiveness in this setting is attributable to model inductive bias and not because of our use of restricted labeling. We leave as an important open question why consistency and restrictiveness are so strongly correlated when training existing models on real-world data.


% \RS{Say that even assuming independence, we can still construct an explicit counterexample. Basically there exists a model that is indistinguishable from the data generated by the data-collection strategy, but which is not disentangled.}

% \RS{if time permits, formalize the impossibility theorem that weak supervision doesn't confer disentanglement? But still have to deal with the issue of independence... For now, don't mention the new flavor of impossibility results.}

% \RS{\citeme{rethinking vae} for rotation experiments.}

% \citeme{all restricted labeling papers that claim disentanglement}
% \loremipsum

==> sections/60_match.tex <==
\subsection{match pairing}

We now consider supervision via match pairing. Formally, we say that a data-collection strategy is match pairing on a subset of factors $I$ if $\strat$ returns the distribution $p_I^*(x, x')$, where $x$ and $x'$ via the process
\begin{align}
    s_I &\sim p^*(s_I)\\
    s_{\sm I}, s_{\sm I}' &\simiid p^*(s_{\sm I} \giv s_I)\\
    (x, x') &= (\gen^*(s_I, s_{\sm I}), \gen^*(s_I, s_{\sm I}')).
\end{align}
In other words, match pairing yields a data distribution over \emph{pairs} of observations that are known to share a set of factors $s_I$. This is a weaker form of supervision than restricted labeling, since the learning algorithm is no longer directly exposed to the underlying label $s_I$. Match pairing is thus more practically feasible; certain variants are already featured in the literature \citeme{multi-level vae, pair-wise similarity, ridgeway, and that obscure match-pair data}. Generally, however, the discussion of match pairing in the literature has centered around \emph{groups} of data that share a \emph{single} factor. We now show that it suffices to deal with pairs of data and formally describe the guarantee of match pairing over multiple factors as follows.

\iffalse
\begin{theorem}\label{thm:match}
Given any oracle $(p^*(s_{1:n}), \gen^*, \enc^*) \in \H$, consider the distribution-matching algorithm $\A$ that selects a model $(p(z_{1:n}), \gen, \enc) \in \H$ such that 
\begin{align}
    \paren{\gen^*(S_I, S_{\sm I}), \gen^*(S_I, S_{\sm I}')}
    \deq 
    \paren{\gen(Z_I, Z_{\sm I}), \gen(Z_I, Z_{\sm I}')}.
\end{align}
Then $\gen$ satisfies $C(I \scolon p, \gen, \enc^*)$ and $\enc$ satisfies $C(I \scolon p^*, \gen^*, \enc)$.
\end{theorem}
\Cref{thm:match} demonstrates that so long as the learning algorithm knows which factors are being shared, match-pairing is sufficient to guarantee consistency on those shared factors. 
\fi

The two most natural forms of match-pairing data are pairs that \emph{share} a single factor $s_i$ and pairs that \emph{change} a single factor $s_i$, which we shall denote as share-pairing and change-pairing. \Cref{thm:match} directly shows that share-pairing guarantees that $z_i$ will be consistent with $s_i$. As for change-pairing, since changing a single factor is equivalent to sharing $s_{\sm I}$, we now apply the calculus ($C(\sm I) \implies R(I)$) to conclude that change-pairing guarantees $z_i$ will be restricted to $s_i$.

To demonstrate the guarantees of \Cref{thm:match} in practice, we trained GANs on all six possible share-pairing setups in Shapes3D, and then measured the normalized consistency and restrictiveness scores respectively. Our results in \Cref{fig:match_share} are consistent with \cref{thm:match}, demonstrating that consistency for factor $s_i$ is highest when the model is explicitly trained on paired data where $s_i$ is shared. We then repeated the same experiment for change-pairing in \Cref{fig:match_change}.

\input{figures/match/boxplot_single_match_shapes3d.tex}

In addition to change and share-pairing experiments, we also trained GANs on \emph{both} change and share-pairing for each factor $s_i$. In \Cref{fig:scatter_cs_shapes3d}, we show scatterplots of consistency versus restrictiveness when trained on either share-pairing, change-pairing, or both for a given factor $s_i$. Interestingly, we can see noticeably in some of the plots that using both types of paired data yields the highest consistency and restrictiveness, whereas training on share-pairing or change-pairing alone only yields the highest consistency or restrictiveness respectively. Similar to what we found in \Cref{fig:label_corrplot}, however, a close inspection of the score ranges ($\ge 0.97$) shows that achieving high restrictiveness and consistency are strongly correlated, and the benefit of training on both share-pairing and change-pairing data---while perhaps statistically significant---is practically negligible. That being said, we do observe in (\Cref{app:match}, \Cref{fig:scatter_cs}) certain situations where training on both is beneficial.

\input{figures/match/scatterplot_cs_shapes3d.tex}

If we have access to share-pairing for each factor (we denote this as \emph{complete-share-pairing}), then our calculus predicts that distribution-matching guarantees full disentanglement. We trained our generative model on the combination of all share-pairing datasets, and measured disentanglement performance via the discretized variant \citep{locatello2018challenging} of the mutual information gap \citep{chen2018isolating}. We then repeated the experiment for change-pairing. As negative and positive controls, we also show the performance of an unsupervised GAN and a fully-supervised GAN. Our results in \Cref{fig:match_mig} empirically verifies that the combination of multiple single-factor pairing datasets leads to a high disentanglement score.

\input{figures/match/boxplot_match_mig.tex}

We now provide a demonstration of the calculus of intersection. In many cases, it may be easier to acquire paired data where multiple factors change simultaneously. Supposing that we have access to two kinds of datasets, one where factors $s_I$ were changed and one where factors $s_J$ were changed, our calculus predicts that training our models on both datasets will guarantee restrictiveness on $s_{I \cap J}$. In \Cref{fig:intersect_main}, we show six such intersection settings and measure the normalized restrictiveness score; in all but one setting, the results are consistent with our theory.

[YC: Why does this one instance fail when we should have guaranteed success?]

\input{figures/match/boxplot_intersect_c.tex}

==> sections/70_rank.tex <==
\subsection{Rank-Pairing}
The last form of supervision we consider 
is rank pairing. Formally, we say that a data-collection strategy is rank pairing on a single factor $s_i$ if $\strat$ returns the distribution $p^*_i(x, x', y)$, where $(x, x', y)$ are sampled via
\begin{align}
    s_{1:n}, s_{1:n}' &\simiid p^*(s_{1:n})\\
    (x, x') &= (\gen^*(s_{1:n}), \gen^*(s_{1:n}'))\\
    y &= \1\set{s_i \ge s_i'}.
\end{align}
In other words, rank pairing yields a data distribution over randomly paired observations $(x, x')$, and then specifies a relation between this pair of observation via an indicator variable $y$ that states whether $s_i \ge s_i'$. Supervision via ranking features prominently in the metric learning literature \citeme{metric learning papers}. In this section, we characterize rank pairing in the context of disentanglement guarantees. 

\iffalse
\begin{theorem}\label{thm:rank}
Given any oracle $p^*(s_{1:n}, \gen^*, \enc^*) \in \H$, consider the distribution-matching algorithm $\A$ that selects a model $(p(z_{1:n}), \gen, \enc) \in \H$ such that
\begin{align}
    \paren{\gen^*(S_{1:n}), \gen^*(S_{1:n}'), \1\set{S_i \le S'_i}}
    \deq 
    \paren{\gen(Z_{1:n}), \gen(Z_{1:n}'), \1\set{Z_i \le Z'_i}}.
\end{align}
Then $\gen$ satisfies $C(I \scolon p, \gen, \enc^*)$ and $\enc$ satisfies $C(I \scolon p^*, \gen^*, \enc)$.
\end{theorem}
\fi

To demonstrate the guarantees of \Cref{thm:rank} in practice, we trained GANs on all six possible rank-pairing setups in Shapes3D, and then measured the normalized consistency scores. Our results in \Cref{fig:single_r_shapes3d} are consistent with \Cref{thm:rank}, demonstrating that consistency for factor $s_i$ is highest when the model is explicitly trained on rank pairing data for $s_i$. Our calculus then predicts that training our models on the complete set of rank pairing datasets yields high disentanglement; we show these results in \Cref{fig:rank_mig}.

\input{figures/rank/boxplot_rank_mig.tex}

% In rank-pairing, we assume that $I$ is a singleton set.
% \subsubsection{Via Distribution Matching}
% \input{figures/rank/boxplot_single_r_shapes3d.tex}
% Consider a data-generating process
% \begin{align}
%     s, s' &\sim p(s)\\
%     (x_d, x_d') &= (\gen^*(s),\gen^*(s'))
% \end{align}
% Consider a model-generating process
% \begin{align}
%     z, z' &\sim p(z)\\
%     (x_g, x_g') &= (\gen(z),\gen(z'))
% \end{align}
% \begin{theorem}
% Under the same assumptions as in section 4, if $(\gen(z),\gen(z'), \mathbf{1}[z <= z']) \stackrel{i.d.}{\sim} (\gen^*(s),\gen^*(s'), \mathbf{1}[s <= s'])$, then $\gen$ satisfies $C_\gen(I)$.
% \end{theorem}
% Let $P(z, z')$ be the property
% \begin{align}
%     z_I<=z_I' \implies \enc_I^* \circ \gen(z_I, z_{\sm I}) <= \enc_I^* \circ \gen(z_I', z_{\sm I}').
% \end{align}
% Crucially, distribution matching guarantees that $\Pr_{z, z'}[P(z, z')] = 1$. 

% Given distribution matching, by symmetry, the encoder is also consistent.
% Consider a data-generating process
% \begin{align}
%     s, s' &\sim p(s)\\
%     (x_d, x_d') &= (\enc(s),\enc(s'))
% \end{align}
% Consider a model-generating process
% \begin{align}
%     z, z' &\sim p(z)\\
%     (x_g, x_g') &= (\enc^*(z),\enc^*(z'))
% \end{align}
% \begin{corollary}
% Under analogous assumptions for encoder $\enc$ as in section 4, if $(\enc^*(z),\enc^*(z'), \mathbf{1}[z <= z']) \stackrel{i.d.}{\sim} (\enc(s),\enc(s'), \mathbf{1}[s <= s'])$, then $\enc$ satisfies $C_\enc(I)$.
% \end{corollary}

% \RS{Move rank prediction to appendix.}

% \subsubsection{Via Rank Prediction}
% Alternatively we can train directly using objective TBA. Suppose training is successful, we have $\Pr_{z, z'}[P(z, z')] = 1$. Therefore generator/encoder consistency follows similarly as in distribution matching.

